A 20-Liter Test Stand with Gas Purification for Liquid Argon Research

We describe the design of a 20-liter test stand constructed to study fundamental properties of liquid argon (LAr). This system utilizes a simple, cost-effective gas argon (GAr) purification to achieve high purity, which is necessary to study electron transport properties in LAr. An electron drift stack with up to 25 cm length is constructed to study electron drift, diffusion, and attachment at various electric fields. A gold photocathode and a pulsed laser are used as a bright electron source. The operational performance of this system is reported.

==> Makefile <==
########################################################################
#
# $Id: Makefile,v 1.2 2010/10/29 15:06:33 slavic Exp $
#
##########################################################################
TEX = pdflatex
BIB = bibtex
#main file
texfile = TS_JINST
#all figures
FIGS=$(wildcard figures/*.*)
#all texfiles
SECS=$(wildcard ./*.tex)
#SECS=$(wildcard sections/*.tex)

export TEXINPUTS:=$(CURDIR):$(CURDIR)/ar2estyle:$(TEXINPUTS)
export BSTINPUTS:=$(CURDIR):$(CURDIR)/ar2estyle:$(BSTINPUTS)
export BIBINPUTS:=$(CURDIR):$(CURDIR)/ar2estyle:$(BIBINPUTS)

.PHONY: pdf
.PHONY: clean

all: pdf

pdf: $(texfile).pdf

$(texfile).pdf : $(SECS) $(texfile).tex $(texfile).bib #$(FIGS) 
	$(TEX) $(texfile)
	$(BIB) $(texfile) # compile bibliography
	$(TEX) $(texfile)
	$(TEX) $(texfile)

clean:
	@ls $(texfile).* | grep -v '.tex\|.bib' | xargs -I {} rm {}

